EasyMimic: A Low-Cost Framework for Robot Imitation Learning from Human Videos

Robot imitation learning is often hindered by the high cost of collecting large-scale, real-world data. This challenge is especially significant for low-cost robots designed for home use, as they must be both user-friendly and affordable. To address this, we propose the EasyMimic framework, a low-cost and replicable solution that enables robots to quickly learn manipulation policies from human video demonstrations captured with standard RGB cameras. Our method first extracts 3D hand trajectories from the videos. An action alignment module then maps these trajectories to the gripper control space of a low-cost robot. To bridge the human-to-robot domain gap, we introduce a simple and user-friendly hand visual augmentation strategy. We then use a co-training method, fine-tuning a model on both the processed human data and a small amount of robot data, enabling rapid adaptation to new tasks. Experiments on the low-cost LeRobot platform demonstrate that EasyMimic achieves high performance across various manipulation tasks. It significantly reduces the reliance on expensive robot data collection, offering a practical path for bringing intelligent robots into homes. Project website: https://zt375356.github.io/EasyMimic-Project/.

==> sec/3_method_revision.tex <==


\section{Method}


%\subsection{Overview}
% 整体流程图

We present \textbf{EasyMimic}, a framework that enables low-cost robots to efficiently leverage human video demonstrations.
The overall framework is illustrated in Figure~\ref{fig:method_overview}.
It consists of three core components: 
1) low-cost collection of both human and robot demonstrations using consumer-grade hardware; 
2) physical alignment across the action and visual domains to bridge the embodiment gap; and 
3) a co-training strategy that effectively fuses human and robot data to train a unified policy model.


\subsection{Data Collection Systems and Hardware Design}

In designing the system, we adhere to the principles of low cost and accessibility.
For the robot platform, we use the LeRobot SO100 manipulator \cite{shukor2025smolvlab,wang2025xlerobot}.
To address the limitations of its original five-degree-of-freedom (5-DoF) design in end-effector orientation control, such as singularities in certain workspace areas that prevent arbitrary poses, we added an extra joint, upgrading it to a six-degree-of-freedom (6-DoF) configuration. 
This extension significantly expands its effective workspace.
We name the upgraded manipulator SO100-Plus.
It has a payload capacity of up to 1 kg and a reach of 400 mm, making it well-suited for various tabletop manipulation tasks.

For data collection, we use a Nintendo Joy-Con for robot teleoperation and deploy two consumer-grade RGB cameras: one fixed in a first-person view (shared by human and robot data collection), and the other mounted on the robot's wrist to capture close-up manipulation details.
The entire system can be assembled for under \$300, far more cost-effective than traditional research platforms.
To process human videos, we leverage the advanced HaMeR model \cite{pavlakos2024reconstructing} to extract 3D hand information from monocular inputs. 
We utilize this model to precisely reconstruct the hand morphology for each video frame, providing 21 hand keypoint coordinates $X_t^\mathcal{C}$ and 778 hand mesh vertex coordinates $V_t^\mathcal{C}$ in the camera coordinate frame $\mathcal{C}$.
This information serves as the foundation for our subsequent alignment process, where keypoints are primarily used for action space mapping and the complete mesh is used for visual space alignment.



\subsection{Physical Alignment} 

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{fig/retargeting_framework.pdf}
    \caption{Physical alignment process. 
        Human hand keypoints and meshes are extracted from videos. Hand motion is retargeted to robot actions via the action space alignment module, while the hand mesh is augmented through the visual space alignment module to bridge the physical gap between humans and robots.}  \label{fig:physical_alignment}
\end{figure}

Human-to-robot transfer requires resolving discrepancies in both kinematics and appearance.
As illustrated in Figure~\ref{fig:physical_alignment}, our alignment module systematically addresses these challenges across action space and visual space.

\subsubsection{Action Space Alignment}
The primary challenge in cross-embodiment imitation is to accurately translate human hand motion trajectories into executable action sequences for the robot's end-effector. 
We need to construct a mapping function from human hand kinematics to robot kinematics.
Given a sequence of human hand keypoints $\mathcal{X}_h = \{X_t\}_{t=1}^T$ extracted from a video, our goal is to generate a corresponding sequence of robot end-effector poses $\mathcal{P}_h = \{P_t\}_{t=1}^T = \{(p_t, q_t, g_t)\}_{t=1}^T$, where $p_t$, $q_t$, and $g_t$ represent its 3D position, orientation (typically as a quaternion or Euler angles), and gripper state, respectively.
This pose sequence constitutes the robot's state representation.

\textbf{Position Alignment:} 
Prior works often use the wrist \cite{liuimmimic} or the midpoint of the fingertips \cite{lepert2025phantomb} as an anchor point, but these can deviate from the true center of interaction during complex manipulations. 
For example, the wrist is too far from the object, while fingertips move relative to each other during fine manipulation, leading to an unstable anchor.
Inspired by unified representation approaches \cite{haldar2025pointb,ren2025motion}, we select the center of the thenar eminence—defined as the midpoint between the thumb's proximal interphalangeal (PIP) joint and the index finger's metacarpophalangeal (MCP) joint—as our retargeting anchor.
This point remains relatively stable during grasping, approximating the palm's center of mass regardless of finger movement. 
It therefore better represents the core region of hand-object interaction.

\textbf{Orientation Alignment:} 
We fit a plane through five keypoints (the four joints of the index finger and the thumb's PIP joint). These five points collectively define the primary orientation of the palm.
The plane's normal vector defines the Z-axis, while the vector from the index finger's MCP to its PIP joint defines the X-axis.
A full 3D coordinate frame is constructed via the cross product, yielding a rotation matrix $R_t$, which is finally converted into the orientation representation $q_t$.

\textbf{Gripper State Alignment:} 
To achieve fine-grained grasping control, we calculate the Euclidean distance $d_t$ between the thumb and index fingertips and normalize it to the range $[0, 1]$ to serve as the gripper state $g_t$:
\begin{equation}
g_t = \text{clip}\left(\frac{d_t - d_{\text{min}}}{d_{\text{max}} - d_{\text{min}}}, 0, 1\right)
\end{equation}
where $d_{\text{min}}$ and $d_{\text{max}}$ are the distance thresholds corresponding to a fully closed and fully open gripper, respectively. 
This continuous gripper state representation, compared to binary open-close control, enables the robot to perform tasks requiring gentle or partial grasps.

After alignment, we use a pre-calibrated hand-eye transformation matrix $T_\mathcal{C}^\mathcal{R}$ to convert the states from the camera frame $\mathcal{P}_h^\mathcal{C}$ to the robot's base frame $\mathcal{P}_h^\mathcal{R}$.
Finally, inspired by chunk-based prediction \cite{zhao2023learningb}, we define the action $a_t$ at timestep $t$ as the state at the next timestep, $P_{h, t+1}$, and form an action chunk $A_t = (a_t, \dots, a_{t+h-1})$ from $h$ future actions. 
% 下面这部分可以删除一些
% This approach provides the policy model with a short-term motion planning horizon, helping to generate smoother and more forward-looking action sequences, effectively reducing the jitter that can arise from frame-by-frame prediction.


\subsubsection{Visual Space Alignment}

The visual discrepancy is another major obstacle in human-to-robot imitation. 
Instead of employing computationally expensive generative models to translate image styles, we propose a lightweight visual augmentation strategy that aligns with the philosophy of our low-cost framework. 
This strategy is based on the idea of domain randomization. Its core objective is to compel the model to ignore task-irrelevant superficial features, such as color and skin texture, and instead learn more fundamental geometric information, such as hand pose and shape.

Specifically, we reuse the extracted 3D hand mesh $M_t$ and render it onto the original image $I_t$. During the rendering process, we apply random color transformations to the entire hand, generating an appearance-standardized augmented view $I_t^{\text{aug}}$. 
By using this augmented data during training, the model is passively exposed to diverse embodiment morphologies. 
% 下面内容可以删掉一些
% This helps the model better adapt to different downstream robot end-effector morphologies. 
This method, without adding any extra complex modules, guides the model at the data level to learn a cross-embodiment visual representation, thereby effectively enhancing its generalization to the robot's morphology. 
% We analyze the effectiveness of this method in our ablation studies.


% 腕部和顶部用view
% 人类和机器人用embodiment
\subsection{Training Strategy}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{fig/trainingstrategy.pdf}
    \caption{Co-training strategy. Human demonstration data and robot teleoperation data are mixed during training. A shared DiT module learns a unified policy representation, while separate action encoders and decoders for each embodiment handle their specific data properties.  }  
    \label{fig:training_strategy}
\end{figure}


To effectively leverage human and robot data, we adopt a co-training strategy. 
These two data sources have complementary advantages: human data is abundant and easy to acquire, containing rich high-level task semantics, while robot data, though scarce, provides precise low-level control signals consistent with its own kinematic properties. 
We combine our processed human demonstration dataset $\mathcal{D}_h$ with a small real-world robot dataset $\mathcal{D}_r$ to form a mixed dataset $\mathcal{D}_{mix}$. 
As shown in Figure~\ref{fig:training_strategy}, all data first passes through a shared frozen vision-language encoder, followed by a shared Diffusion Transformer (DiT) module for cross-embodiment policy learning.

In our implementation, to handle data imbalance, we use balanced sampling to ensure that each minibatch contains data from both human and robot sources. 
As the human videos lack the wrist-mounted camera view, we apply zero-padding to the corresponding image data to maintain consistent input dimensions.

Furthermore, while the core DiT module is shared, we design independent encoders and decoders for the state ($P_t$) and the noised action ($A_n$) for each embodiment (human and robot). 
% 下面这部分可以删掉一些
This design allows the model to flexibly handle differences in dimensionality, numerical ranges, and physical meanings between the two data types, leading to a more stable shared policy learning process. 
% In this way, the model can learn generalizable task knowledge from abundant human data while simultaneously being ``calibrated" and ``grounded" by a small amount of precise robot data to learn robot-specific low-level control details.






==> sec/4_exp_bak.tex <==





\section{Experiment}

\subsection{Experimental Setup}
% 我们使用lerobot_plus机械臂作为实验平台，配备了一个夹爪作为末端执行器。使用单目RGB相机作为全局视角输入，摄像头安装在机械臂基座上方，俯视拍摄操作区域。同时使用腕部相机作为近距离视角输入，摄像头安装在机械臂末端夹爪上。使用Groot作为基础模型，训练和推理时使用绝对动作表示。我们设计了3个不同类型的桌面常见任务，每个任务中进行了10次独立的试验，以评估机器人的性能。

% 参考文献连续编号

We use the lerobot\_plus robotic arm with a gripper as end-effector. Two monocular RGB cameras provide visual input: a top-down camera mounted above the base and a wrist camera on the gripper. We employ Gr00t n1.5-3B as the foundation model with absolute action representation. We design three different types of common desktop tasks, conducting 10 independent trials for each task to evaluate the robot's performance.

\subsection{Tasks Descriptions}

\subsubsection{Pick and Place} The robot picks up a duck and place it into a designated bowl. A successful pick earns 0.5 points, and a successful place earns another 0.5, for a total of 1 point.

\subsubsection{Pull and Push} The robot is tasked with opening a drawer and then pushing it closed. Success is scored with 0.5 points for opening and 0.5 points for closing, totaling 1 point.

% 补充数据收集用时的表格，考虑一下要不要加，使用插值前的数据时间
\begin{table}[htbp]
    \centering 
    \begin{tabular}{c c c c c c c}
        \toprule
        Task & \multicolumn{3}{c}{H} & \multicolumn{3}{c}{R} \\
        \cmidrule(lr){2-4} \cmidrule(lr){5-7}
             & \# & min & \#/min & \# & min & \#/min \\
        \midrule
        Pick and Place & 100 & 8.3 & 12 & 20 & 10 & 2 \\
        Pull and Push & 100 & 10 & 10 & 20 & 15 & 1.3 \\
        \bottomrule
    \end{tabular}
        \caption{Data collection overview. The table shows the number of demonstrations (\#), collection time (min), and collection rate (\#/min) for both human (H) and robot (R) data across different tasks.}  
        \label{tab:data_collection}
\end{table}


% \subsubsection{Pick and Place with Language Prompt}In this task, we evaluate the robot's ability to perform out-of-distribution (OOD) generalization by providing a language prompt: "Pick up the pink/green/othercolor duck and place it in the bowl." This requires the robot to not only understand the instruction but also to identify and interact with objects based on color, demonstrating its ability to generalize to unseen object properties. The robot must interpret the instruction and execute the task accordingly, showcasing its language understanding and adaptability.

\subsection{Experimental Results}

\subsubsection{Effect of Training Strategy}
We evaluate three training strategies: training solely on robot data, pre-training on human data before fine-tuning on robot data and co-training with both human and robot data. As shown in~\autoref{Evaluate Training Strategies}, incorporating human demonstrations via co-training or pre-training significantly improves performance over using only robot data. This suggests that human data enhances the model's generalization and task execution. Furthermore, co-training occasionally surpasses pre-training, possibly by better leveraging the diversity in human data.

% 下面这个表格， R 10 + H 50 条  
%only robot: 3/10
%R 10 + H 25 -cotraining : 8.5/10
%R 10 + H 50 -cotraining : 10/10
%R 10 + H 50 -pretrained : 8/10


\begin{table}[htbp]
    \centering 
    \begin{tabular}{c c c c}
        \toprule
        Strategy         & Pick and place & Pull and Push & \\
        \midrule
        Only Robot (10)      &    3/10       &  3/10 \\
        Only Robot (20)      &    6/10       & 7/10  \\
        Pretrain-finetune    &    8/10      &  9/10 \\
        Co-training  &      \textbf{10/10}       & \textbf{10/10}\\
        \bottomrule
    \end{tabular}
    \caption{Evaluate Training Strategies}
\end{table}

% cotraining 10 + 50 Human : 8/10
% cotraining 10 + 100 Human : 9.5/10 
% pretain 10 + 50 Human : 9.5/10

% 使用共享的动作头（NN）和独立的动作头（RH）对模型性能的影响。从表X中可以看出，使用独立动作头（RH）的模型在大多数任务中表现优于使用共享动作头（NN）的模型。这可能是因为独立动作头能够更好地适应不同数据源（机器人和人类）的特性，从而提升模型的任务执行能力。


\subsubsection{Effect of Dataset Size}
% 我们评估了不同规模的人类演示数据对模型性能的影响。从图X中可以看出，随着人类数据规模的增加，模型在所有任务中的表现都有显著提升。结合具体数值。这可能是由于人手数据提供了更多样化的示例和更丰富的任务信息，从而帮助模型更好地理解任务要求和环境特征，提高其泛化能力。此外，我们还比较了在相同人类数据规模下，不同机器人数据规模对模型性能的影响。从表X中可以看出，仅需较少的机器人数据，结合大量人类数据，模型就能达到较好的性能。结合具体数值。
We evaluate the impact of varying amounts of human demonstration data on model performance. As shown in~\autoref{fig:dataset_size}, the model's performance across all tasks improves significantly as the scale of human data increases. This improvement can be attributed to the human hand data providing more diverse examples and richer task information, thereby helping the model better understand task requirements and environmental features, ultimately enhancing its generalization capability. Additionally, we compare the effect of different robot data scales on model performance while keeping the human data scale constant. The results demonstrate that with only a small amount of robot data combined with substantial human data, the model can achieve satisfactory performance.

\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{0.48\linewidth}
        \includegraphics[width=\linewidth]{fig/human_number.pdf}
        \caption{}
        \label{fig:human_dataset_size}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\linewidth}
        \includegraphics[width=\linewidth]{fig/robot_number.pdf}
        \caption{}
        \label{fig:robot_dataset_size}
    \end{subfigure}
    \caption{Effect of Dataset Size. (a) Varying the amount of human data while keeping the robot data fixed. (b) Varying the amount of robot data while keeping the human data fixed.}
    \label{fig:dataset_size}
\end{figure}


\subsubsection{Effect of Human Data Retargeting}
% 我们评估了对人类演示数据进行动作空间对齐（retargeting）以及视觉增强对模型性能的影响。从图x中可以看出，进行动作空间对齐的模型在大多数任务中表现优于不进行对齐的模型。这可能是因为动作空间对齐有助于减少人类和机器人数据之间的差异，使模型更容易学习到通用的任务表示和策略，从而提升其任务执行能力。

% baseline-AA 表示使用腕部对齐替代手掌虎口对齐，baseline-VA表示不进行人类演示数据视觉增强，


\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.8\linewidth]{fig/retargeting.pdf}
    \caption{Effect of Human Data Retargeting. AA: action space alignment; VA: visual augmentation.}
    \label{fig:enter-label}
\end{figure}


\subsubsection{Effect of text prompt Augmentation}
% 我们评估了在文本中显式添加具身描述如[Human]和[robot]对模型性能的影响。从表X中可以看出，添加具身描述的文本提示显著提升了模型在所有任务中的表现。这表明具身描述有助于模型更好地理解任务要求和环境信息，从而提高其任务执行能力。

\begin{table}[htbp]
    \centering 
    \begin{tabular}{c c c c}
        \toprule
        Strategy         & Pick and place & Pull and Push \\
        \midrule
        Baseline    &    \textbf{10/10}      &  \\
        W/o text prompt Augmentation  &         &  \\
        \bottomrule
    \end{tabular}
    \caption{Effect of text prompt Augmentation}
\end{table}


% 这一部分检验模型的泛化能力。我们设计了一个新的任务“Pick and Place with Language Prompt”，要求机器人根据语言提示选择特定颜色的y鸭子以及物体进行抓取和放置。通过在文本提示中加入颜色信息，评估模型在处理未见过的物体属性时的表现。实验结果表明，模型能够成功理解并执行基于颜色的指令，展示了其在语言理解和任务适应方面的能力。
\subsubsection{Generalization Evaluation}
We evaluate the model's generalization capability through two aspects: color generalization and object generalization. For color generalization, we provide language prompts such as "Pick up the pink/green/blue duck and place it in the bowl," requiring the robot to identify and interact with objects based on specified colors. For object generalization, we test the model's ability to handle different objects beyond the training data, demonstrating its adaptability to novel items.

\begin{table}[htbp]
    \centering 
    \begin{tabular}{c c c c}
        \toprule
        Strategy         & Color Generalization & Object Generalization \\
        \midrule
        Baseline    &          &         $\times$ \\
        \bottomrule
    \end{tabular}
    \caption{Generalization Evaluation}
\end{table}


% \subsection{0830 Experiment Results}

% Use the \textbf{top view} camera to do the evaluation, including the training and inference.
% Co-training and Pretrain-finetune means 10 Robot data + 50 Human data.

% \begin{table}[htbp]
%     \centering 
%     \begin{tabular}{c c c c}
%         \toprule
%         Strategy         & Pick and place & Done & \\
%         \midrule
%         Only Robot (5)       &    0/10       & $\checkmark$  \\
%         Only Robot (10)       &    3/10       & $\checkmark$  \\
%         Only Robot (20)       &     6/10       & $\checkmark$  \\
%         Co-training (w/ retargeting)(RR)      &            & $\times$ \\
%         Co-training (w/ retargeting)(RH)      &            & $\times$ \\
%         Pretrain-finetune (w/ retargeting)(RR) &            & $\times$ \\
%         Pretrain-finetune (w/ retargeting)(RH) &            & $\times$ \\
%         \bottomrule
%     \end{tabular}
%     \caption{Evaluate Training Strategies}
% \end{table}

% \subsection{0831 Experiment Results}

% \begin{table}[htbp]
%     \centering
%     \begin{tabular}{c c c c}
%         \toprule
%         Strategy         & Pick and place & Done & \\
%         \midrule
%         Co-training (w/ retargeting)($R_{10},H_0$)       &            & $\times$ \\
%         Co-training (w/ retargeting)($R_{10},H_{25}$)       &            & $\times$ \\
%         Co-training (w/ retargeting)($R_{10},H_{50}$)       &            & $\times$ \\
%         Co-training (w/ retargeting)($R_{10},H_{100}$)       &            & $\times$ \\
%         Co-training (w/ retargeting)($R_{1},H_{100}$)       &            & $\times$ \\
%         Co-training (w/ retargeting)($R_{5},H_{100}$)       &            & $\times$ \\
%         \bottomrule
%     \end{tabular}
%     \caption{Evaluate data size (human, robot)}
% \end{table}



% \subsection{0901 Experiment Results}

% \begin{table}[htbp]
%     \centering
%     \begin{tabular}{c c c c}
%         \toprule
%         Strategy         & clean the table & Done & \\
%         \midrule
%         Only Robot (5)       &          & $\times$  \\
%         Only Robot (10)       &          & $\times$  \\
%         Only Robot (20)       &           & $\times$  \\
%         Co-training (w/ retargeting)(RR)      &            & $\times$ \\
%         Co-training (w/ retargeting)(RH)      &            & $\times$ \\
%         Pretrain-finetune (w/ retargeting)(RR) &            & $\times$ \\
%         Pretrain-finetune (w/ retargeting)(RH) &            & $\times$ \\
%         \bottomrule
%     \end{tabular}
%     \caption{Evaluate training strategies for the Clear the Table task}
% \end{table}


% \begin{table}[htbp]
%     \centering
%     \begin{tabular}{c c c c}
%         \toprule
%         Strategy         & Pick and place & Done  \\
%         \midrule
%         Co-training (w/o retargeting)(RH)      &            & $\times$ \\
%         Pretrain-finetune (w/o retargeting)(RH) &            & $\times$ \\
%         \bottomrule
%     \end{tabular}
%     \caption{0830 Experiment Results A}
% \end{table}


% \begin{table}[htbp]
%     \centering
%     \begin{tabular}{c c c}
%         \toprule
%         Strategy         & Pick and place & Done \\
%         \midrule
%         w/o action space alignment(?)       & 0.00           & $\times$ \\
%         Thenar space alignment & 0.00           & $\times$ \\
%         Wrist alignment       & 0.00           & $\times$ \\
%         \bottomrule
%     \end{tabular}
%     \caption{0830 Experiment Results B}
% \end{table}





% \subsubsection{results}


% \begin{table}[htbp]
%     \centering
%     \begin{tabular}{c c c c}
%         \toprule
%         Strategy         & Pick and place & Clear the table & Put the pen\\
%         \midrule
%         Only Robot (5)       & 0/10           & 0 & 0 \\
%         Only Robot (10)       & 3/10           & 0 & 0 \\
%         Only Robot (20)       & 6/10           & 0 & 0 \\
%         Co-training (w/ retargeting)(NN)      & 0           & 0 & 0\\
%         Co-training (w/ retargeting)(RH)      & 0           & 0 & 0\\
%         Co-training (w/o retargeting)(RH)      & 0           & 0 & 0\\
%         Pretrain-finetune (w/ retargeting)(NN) & 0           & 0 & 0\\
%         Pretrain-finetune (w/ retargeting)(RH) & 0           & 0 & 0\\
%         Pretrain-finetune (w/o retargeting(RH))& 0           & 0 & 0\\
%         \bottomrule
%     \end{tabular}
%     \caption{Training strategies}
%     \label{tab:results_strategy_a}  
% \end{table}




% \begin{table}[htbp]
%     \centering
%     \begin{tabular}{c c c}
%         \toprule
%         Strategy         & Pick and place & Push \\
%         \midrule
%         Only Robot (R)       & 0/10           & 0 \\
%         Co-training (w/ retargeting)(NN)      & 0/10          & 0 \\
%         Co-training (w/ retargeting)(RH)      & 2+0.5+0.5/10           & 0 \\
%         Co-training (w/o retargeting)(RH)      & 0/10           & 0 \\
%         Pretrain-finetune (w/ retargeting)(NN) &      0/10      & 0 \\
%         Pretrain-finetune (w/ retargeting)(RH) & 0.5+0.5/10 & 0 \\
%         Pretrain-finetune (w/o retargeting(RH))&    0        & 0 \\
%         \bottomrule
%     \end{tabular}
%     \caption{Training strategies}
%     \label{tab:results_strategy_a}  
% \end{table}

% % 0820update
% 10 trials, each lasting 80s, with multiple attempts allowed within each trial. The small bowl is fixed, and the pink duck is manually placed in 3 initial positions (3/3/4) in an L-shape for each trial. Experimental results indicate that, during inference, the robotic arm achieves its best performance at the rightmost test point within the L-shaped test range.
% \begin{table}[htbp]
%     \centering
%     \begin{tabular}{ll}
%         \toprule
%         Parameter                      & Value         \\
%         \midrule
%         Robot data size                & 30 examples   \\
%         Human data size                & 100 examples  \\
%         Hand video interpolation/ Hand video flicker         & 4/2           \\
%         Hand action space alignment    & Thenar        \\
%         Hand visual augmentation       & Full hand     \\
%         Data preprocessing            & min-max(mixed process) \\
%         \bottomrule
%     \end{tabular}
%     \caption{Experimental Parameters}
%     \label{tab:parameters}
% \end{table}

% NN, RH represent the action heads. NN denotes using the same action head "new\_embodied". RH denotes using different action heads "lerobot\_plus" and "human\_hand" for robot and human data respectively.



% % 数据集问题！！没有正确更新数据集的metadata status.json
% % 在Pretrain-finetune (w/o retargeting) 中第一条正确抓取，但是没有成功放置，后续4条在某个位置（0.22，0.08，0.189，1.5，0.47，0.1，10）附近小幅度抖动，且移动物体没用明显响应

% \begin{table}[htbp]
%     \centering
%     \begin{tabular}{c c c}
%         \toprule
%         Strategy         & Pick and place & Push \\
%         \midrule
%         No augmentation       & 0.00           & 0.00 \\
%         Full hand       & 0.00           & 0.00 \\
%         Index finger and thumb      & 0.00           & 0.00 \\
%         Index finger and thumb (joint)& 0.00           & 0.00 \\
%         \bottomrule
%     \end{tabular}
%     \caption{Human hand visual color augmentation}
%     \label{tab:results_strategy_b}  
% \end{table}


% \begin{table}[htbp]
%     \centering
%     \begin{tabular}{c c c}
%         \toprule
%         Strategy         & Pick and place & Push \\
%         \midrule
%         w/o action space alignment       & 0.00           & 0.00 \\
%         Thenar space alignment & 0.00           & 0.00 \\
%         Wrist alignment       & 0.00           & 0.00 \\
%         \bottomrule
%     \end{tabular}
%     \caption{Human-Robot action space alignment}
%     \label{tab:results_strategy_c}  
% \end{table}

% Note that ``Thenar space alignment" in \ref{tab:results_strategy_c} refers to aligning the action space of the palm's muzzle to the robot's action space, while ``Wrist alignment" refers to aligning the wrist's action space to the robot's action space. While ``w/o action space alignment" is the case where no calibration is performed.


% \begin{table}[htbp]
%     \centering
%     \begin{tabular}{c c c}
%         \toprule
%         Strategy         & Pick and place & Push \\
%         \midrule
%         Text augmentation        & 0.00           & 0.00 \\
%         Freeze vit and llm  & 0.00           & 0.00 \\
%         State action augmentation       & 0.00           & 0.00 \\
%         Visual augmentation       & 0.00           & 0.00 \\
%         \bottomrule
%     \end{tabular}
%     \caption{Training augmentation in Gr00t}
%     \label{tab:results_strategy_c}  
% \end{table}
















% 我们评估了对人类演示数据进行动作空间对齐（retargeting）以及视觉增强对模型性能的影响。从图x中可以看出，进行动作空间对齐的模型在大多数任务中表现优于不进行对齐的模型。这可能是因为动作空间对齐有助于减少人类和机器人数据之间的差异，使模型更容易学习到通用的任务表示和策略，从而提升其任务执行能力。

% baseline-AA 表示使用腕部对齐替代手掌虎口对齐，baseline-VA表示不进行人类演示数据视觉增强，


% 我们评估了在文本中显式添加具身描述如[Human]和[robot]对模型性能的影响。从表X中可以看出，添加具身描述的文本提示显著提升了模型在所有任务中的表现。这表明具身描述有助于模型更好地理解任务要求和环境信息，从而提高其任务执行能力。

% \begin{table}[htbp]
%     \centering 
%     \begin{tabular}{c c c c}
%         \toprule
%         Strategy         & Pick and place & Pull and Push \\
%         \midrule
%         Baseline    &    \textbf{10/10}      &  \\
%         W/o text prompt Augmentation  &         &  \\
%         \bottomrule
%     \end{tabular}
%     \caption{Effect of text prompt Augmentation}
% \end{table}


% 这一部分检验模型的泛化能力。我们设计了一个新的任务“Pick and Place with Language Prompt”，要求机器人根据语言提示选择特定颜色的y鸭子以及物体进行抓取和放置。通过在文本提示中加入颜色信息，评估模型在处理未见过的物体属性时的表现。实验结果表明，模型能够成功理解并执行基于颜色的指令，展示了其在语言理解和任务适应方面的能力。
% \subsubsection{Generalization Evaluation}
% We evaluate the model's generalization capability through two aspects: color generalization and object generalization. For color generalization, we provide language prompts such as "Pick up the pink/green/blue duck and place it in the bowl," requiring the robot to identify and interact with objects based on specified colors. For object generalization, we test the model's ability to handle different objects beyond the training data, demonstrating its adaptability to novel items.

% \begin{table}[htbp]
%     \centering 
%     \begin{tabular}{c c c c}
%         \toprule
%         Strategy         & Color Generalization & Object Generalization \\
%         \midrule
%         Baseline    &          &         $\times$ \\
%         \bottomrule
%     \end{tabular}
%     \caption{Generalization Evaluation}
% \end{table}



% \subsubsection{Effect of Language Prompts}
% We ablate the use of domain-specific prompts (\texttt{[Human]} and \texttt{[Robot]}). 
% As shown in Table~\ref{tab:prompt_ablation}, removing these prompts causes a significant drop in performance. 
% This indicates that the prompts serve as crucial domain identifiers that help the model avoid policy confusion.

% \begin{table}[h]
%     \centering 
%     \begin{tabular}{l c c c c}
%         \toprule
%         \textbf{Strategy} & \textbf{Pick} & \textbf{Pull} & \textbf{Stack} & \textbf{Avg.} \\
%         \midrule
%         \textbf{With Prompts} & \textbf{1.00}  & \textbf{0.90} & \textbf{0.70} & \textbf{0.83} \\
%         Without Prompts & 0.90 & 0.80 & 0.60 & 0.70  \\
%         \bottomrule
%     \end{tabular}
%     \caption{Ablation on the effect of domain-specific language prompts.}
%     \label{tab:prompt_ablation}
% \end{table}
